Fool Me Twice: Entailment from Wikipedia Gamification

We release FoolMeTwice (FM2 for short), a large dataset of challenging entailment pairs collected through a fun multi-player game. Gamification encourages adversarial examples, drastically lowering the number of examples that can be solved using "shortcuts" compared to other popular entailment datasets. Players are presented with two tasks. The first task asks the player to write a plausible claim based on the evidence from a Wikipedia page. The second one shows two plausible claims written by other players, one of which is false, and the goal is to identify it before the time runs out. Players "pay" to see clues retrieved from the evidence pool: the more evidence the player needs, the harder the claim. Game-play between motivated players leads to diverse strategies for crafting claims, such as temporal inference and diverting to unrelated evidence, and results in higher quality data for the entailment and evidence retrieval tasks. We open source the dataset and the game code.

==> 2020_tacl_factcheck/sections/70-human_computer.tex <==
\input{2020_tacl_factcheck/tables/accuracy}

\subsection{Human--Computer Competition}
\label{sec:human-computer}

% All of these results with respect to BERT model

There is substantial correlation in accuracy between human and computers.  
%
Humans have 0.82 accuracy on claims the model get right but 0.74 on claims the model gets wrong.
%
However, there are divergences; let's take a closer look at which ones.

Our two-phase data generation process is not just to generate more challenging claims.
%
It can also provide a comparison between human and computer claim entailment. 
%
This section examines which claims are more difficult for computers or vice-versa.




% Examples of false claims they did like





==> 2020_tacl_factcheck/tables/accuracy.tex <==
\begin{table*}[]
    \centering
    \begin{small}
    \begin{tabular}{lccccc}
    \toprule
        & \multicolumn{5}{c}{Human accuracy} \\
        & $[0,0.25]$ & $[0.25,0.5]$ & $[0.5,0.75]$ & $[0.75,1.0)$ & $1.0$ \\
        \midrule
        Computer Correct & 0.01 & 0.03 & 0.18 & 0.14 & 0.37 \\
        Computer Wrong & 0.01 & 0.02 & 0.08 & 0.05 & 0.10 \\
        \bottomrule
    \end{tabular}
    \end{small}
    \caption{Comparing computer accuracy to human accuracy (proportion of voters who selected the true false claim).  }
    \label{tab:accuracy}
\end{table*}
